Quantum spectral curve for the $\eta$-deformed AdS$_5 \times $S$^5$ superstring

In this thesis we discuss how one can derive the quantum spectral curve for the $\eta$-deformed AdS$_5 \times S^5$ superstring, an integrable deformation of the AdS$_5 \times $S$^5$ superstring with quantum group symmetry. This model can be viewed as a trigonometric version of the AdS$_5 \times $S$^5$ superstring, like the Heisenberg xxz spin chain is a trigonometric version of the xxx spin chain. Our derivation starts from the ground-state thermodynamic Bethe ansatz equations and discusses the construction of both the undeformed and the $\eta$-deformed quantum spectral curve. We reformulate it first as an analytic $Y$-system, and map this to an analytic $T$-system which upon suitable gauge fixing leads to a $\mathbf{P}\mu$ system, the quantum spectral curve. We then discuss constraints on the asymptotics of this system to single out particular excited states. At the spectral level the $\eta$-deformed string and its quantum spectral curve interpolate between the AdS$_5 \times $S$^5$ superstring and a superstring on "mirror" AdS$_5 \times $S$^5$, reflecting a more general relationship between the spectral and thermodynamic data of the $\eta$-deformed string. The thesis is set up such that it simultaneously reviews the development of the undeformed AdS$_5 \times $S$^5$ quantum spectral curve.

==> Yvwdisc.tex <==
The $Y_{M|vw}$ functions do not have a discontinuity on the real line, and the only $Y_{M|vw}$ with a discontinuity at $\pm 1$ is  $Y_{1|vw}$, for which we have \eqref{discs1}. Taking logs of the $Y$-system equations \eqref{eq:Ysystem} for $Y_{M|(v)w}$ we find for $M\geq 2$
\be
\log Y_{M|vw}^+ +\log Y_{M|vw}^- =\sum_{N=1}^{\infty} A_{MN} \Lambda_{N|vw}-\Lambda_{M+1},
\ee
with $A_{MN}$ as in \eqref{eq:AMJ}. Taking discontinuity brackets at $M+2l-1$ yields
\bea
\label{hulpje1v}
& &\left[ \log Y_{M|vw} \right]_{M+2l} =  \sum_{N=1}^{\infty} A_{MN} \left[L_{N|vw}\right]_{M+2l -1} +  \left[\log Y_{M-1|vw}\right]_{M+2l-1} + \left[\log Y_{M+1|vw}\right]_{M+2l-1} \nn 
&-&\left[\Lambda_{M+1}\right]_{M+2l-1} - \left[\log Y_{M|vw}\right]_{M+2(l-1)}. 
\eea
This is the rule that we can use repeatedly to bring the discontinuity containing $\log Y_{Q|vw}$ () closer and closer to the real line

Using the second line of \eqref{hulpje1v} first yields: 
\bea 
& &\left[ \log Y_{M|vw} \right]_{M+2l} = \nonumber \\
&=&\sum_{N=1}^{\infty}  A_{MN} \left[L_{N|vw}\right]_{M+2l -1} +  \left[\log Y_{M-1|vw}\right]_{M+2l-1} + \left[\log Y_{M+1|vw}\right]_{M+2l-1} -\left[ \log Y_{M|vw} \right]_{M+2l-2}\nonumber \\
&-&\left[\Lambda_{M+1}\right]_{M+2l-1} \nn
&=& \sum_{N=1}^{\infty}  A_{MN} \left[L_{N|vw}\right]_{M+2l -1} + \sum_{N=1}^{\infty}  A_{M-1,N} \left[L_{N|vw}\right]_{M-1+2l -1} -\left[ \log Y_{M|vw} \right]_{M+2l-2}\nonumber \\ 
&+&  \left[\log Y_{M-2|vw}\right]_{M+2l-2} +\left[\log Y_{M|vw}\right]_{M+2(l-1)} + \left[\log Y_{M+1|vw}\right]_{M+2l-1}-\left[\log Y_{M-1|vw}\right]_{M+2l-3} \nn
&-&\left[\Lambda_{M+1}\right]_{M+2l-1} - \left[\Lambda_{M}\right]_{M-1+2l-1}, \nn 
\eea
so we can conclude that 
\bea 
& &\left[ \log Y_{M|vw} \right]_{M+2l} -\left[\log Y_{M+1|vw}\right]_{M+2l-1} = \nonumber \\
&=& \sum_{Q=M-1}^M \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -1}+  \left[\log Y_{M-2|vw}\right]_{M+2l-2}-\left[\log Y_{M-1|vw}\right]_{M+2l-3}-\sum_{Q=M}^{M+1} \left[\Lambda_Q\right]_{Q+2l-2}.\nn
\eea
Repeated application now leads to the result
\bea
\label{rep1v}
& &\left[ \log Y_{M|vw} \right]_{M+2l} -\left[\log Y_{M+1|vw}\right]_{M+2l-1} = \nonumber \\
&=&\sum_{Q=2}^M \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -1}+  \left[\log Y_{1|vw}\right]_{1+2l}-\left[\log Y_{2|vw}\right]_{2l}-\sum_{Q=3}^{M+1} \left[\Lambda_Q\right]_{Q+2l-2}.
\eea
Plugging in the Y-system equation for $Y_{1|vw}$ gives us
\bea
\label{rep2v}
& &\left[ \log Y_{M|vw} \right]_{M+2l} -\left[\log Y_{M+1|vw}\right]_{M+2l-1} = \nonumber \\
&=&\sum_{Q=2}^M \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -1}-  \left[\log Y_{1|vw}\right]_{1+2l-2} +\left[L_{2|vw}\right]_{2l}+\left[\Lambda_--\Lambda_+ \right]_{2l}-\sum_{Q=2}^{M+1} \left[\Lambda_Q\right]_{Q+2l-2}. \nonumber \\
&=&\sum_{Q=1}^M \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -1}-  \left[\log Y_{1|vw}\right]_{1+2l-2} +\left[\Lambda_--\Lambda_+ \right]_{2l}-\sum_{Q=2}^{M+1} \left[\Lambda_Q\right]_{Q+2l-2}. \nonumber \\
\eea
The addition of the sum over $\Lambda_Q$ is the only difference with the $Y_w$-case. The derivation below is therefore completely analogolous to the $Y_w$-case. 
\\[5mm]
Using the line \eqref{rep1v} with first term $\left[ \log Y_{M+1|vw} \right]_{M+2l-1}$ (So $M\rightarrow M+1,l\rightarrow l-1$) gives 
\bea
& &\left[ \log Y_{M+1|vw} \right]_{M+2l-1} = \left[\log Y_{M+2|vw}\right]_{M+2l-2}  \nonumber \\
&+&\sum_{Q=2}^{M+1} \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -3}+  \left[\log Y_{1|vw}\right]_{2l-1}-\left[\log Y_{2|vw}\right]_{2l-2}-\sum_{Q=3}^{M+2} \left[\Lambda_Q\right]_{Q+2l-4}.
\eea
Note the existence of a term $\left[\log Y_{1|vw}\right]_{2l-1}$ in \eqref{rep2v} and also in the last line. When combining the statements, these terms will cancel. We can repeatedly do this to end up with
\bea
\label{resvw1}
& &\left[ \log Y_{M|vw} \right]_{M+2l} = \left[ \log Y_{M+l+1|vw} \right]_{M+l-1} -\sum_{J=1}^{l+1}\sum_{Q=1+J}^{M+J} \left[\Lambda_Q\right]_{Q+2l-2J} \nn
&+&\sum_{J=0}^l\sum_{Q=1+J}^{M+J} \sum_{N=1}^{\infty}  A_{QN} \left[L_{N|vw}\right]_{Q+2l -1-2J} + \left[\Lambda_--\Lambda_+\right]_{2l} -\left[\log Y_{l+1|vw}\right]_{l-1},
\eea
where the first and last term usually vanish because of the fact that the functions in the brackets are analytic on the respective strips (except at the very important exception $l=0$, for which the last term does contribute). The expression only differs from the one for $Y_w$ because of the addition of the sums over $\Lambda_Q$, in which we will drop the term corresponding to $J=l+1$ because the summands vanish. In particular the triple sum is completely the same as the one for $Y_w$, allowing us to use the expression derived in \eqref{longder1} where all we need to do is replace $Y_w\rightarrow Y_{vw}$. This leads to the result
\bea
& &\left[ \log Y_{M|vw} \right]_{M+2l} =  \left[\Lambda_--\Lambda_+  \right]_{2l} -\delta_{l,0}\left[\Lambda_-\right]_0 -\sum_{J=1}^{l}\sum_{Q=1+J}^{M+J} \left[\Lambda_Q\right]_{Q+2l-2J}\nn
&+& \sum_{J=1}^l \left( 2 \sum_{Q=1}^{M-1}  \left[L_{Q+J|vw}\right]_{Q+2l-J} + \left[L_{M+J|vw}\right]_{M+2l-J}\right)+\sum_{Q=1}^{M-1} \left[L_{Q|vw}\right]_{Q+2l } +  \sum_{J=1}^l   \left[L_{J|vw}\right]_{2l-J}.\nonumber \\
\eea
We define the discontinuities completely analogously to last time
\bea
\left[D^{M|vw}_{M+2l}\right]_0(u) &=&\left[\Lambda_--\Lambda_+ \right]_{2l} +\sum_{Q=1}^{M-1} \left[L_{Q|vw}\right]_{Q+2l } +  \sum_{J=1}^l   \left[L_{J|vw}\right]_{2l-J} \nn
&+& \sum_{J=1}^l \left( 2 \sum_{Q=1}^{M}  \left[L_{Q+J|vw}\right]_{Q+2l-J} + \left[L_{M+J|vw}\right]_{M+2l-J}\right)-\sum_{J=1}^{l}\sum_{Q=1+J}^{M+J} \left[\Lambda_Q\right]_{Q+2l-2J},\nn
\eea
where the $D$ themselves can be identified in a straightforward way with the arguments of the brackets. We have the following identity that is just an extended version of the one we had for $Y_w$:
\bea
\label{Didentityv}
D^{M|vw}_{(M+2l)\tau }(u) - D^{M|vw}_{\tau(M+2l-2)}(u+\tau 2i a ) &=& L_{l|vw}(u+\tau li a)+L_{M+l|vw}(u+\tau (M+l)i a ) \nn
&+& 2 \sum_{Q=l+1}^{M-1+l}  L_{Q|vw}(u+\tau Qai) -\sum_{Q=1+l}^{M+l} \Lambda_Q(u+\tau Qai), \nn
\eea
Now we can plug this into our Cauchy integral expression for $\log Y_{vw}$: 
\bea
\label{92v}
& &\sum_{\tau}\sum_{l=0}^{\infty} \left( \int_{(-\pi,\pi) +\tau(M+2l) +i\e} -\int_{(-\pi,\pi)+\tau(M+2l) -i\e} \right)  \log Y_{M|vw}(z) H(z-u) \nn
&=&\sum_{\tau}\sum_{l=0}^{\infty} \int  \left[\log Y_{M|vw}\right]_{\tau (M+2l)}(z) H(z+\tau (M+2l)-u) \nn
&=&\sum_{\tau}\sum_{l=0}^{\infty} \int \left(\left[D_{(M+2l)\tau }^{M|vw}\right]_{0}(z) -\delta_{l,0}\left[\Lambda_-\right]_0  \right) H(z+\tau (M+2l) -u) \nn
&=& - \left(\int_{(-\pi,\pi)+i\e}-\int_{(-\pi,\pi)-i\e}\right)\left(\Lambda_-(z) H(z+M a i -u) + \Lambda_-(z) H(z-M a i -u)\right) \nn
&+& \sum_{\tau}\sum_{l=0}^{\infty} \int \left(\left[D_{(M+2l)\tau}^{M|vw}\right]_{0}(z) \right) H(z+\tau (M+2l)-u) .
\eea
The last integrals are again very similar to the ones we used for $Y_w$, so we see immediately that
\bea
\label{93v}
& & \sum_{\tau}\sum_{l=0}^{\infty} \int \left(\left[D_{(M+2l)\tau}^{M|vw}\right]_{0}(z) \right) H(z+\tau (M+2l)-u) \nn
&=&  - \sum_{\tau}\sum_{l=1}^{\infty}\tau  \int_{(-\pi,\pi) -i\tau \e } \left(D_{(M+2l)\tau}^{M|vw}(z) -D_{(M+2l-2)\tau}^{M|vw}(z+2\tau a)\right) H(z+\tau (M+2l)a-u) \nn
&-&\sum_{\tau} \tau \int_{(-\pi,\pi) -i\tau \e }\left(\left(\Lambda_--\Lambda_+ \right) + \sum_{Q=1}^{M-1} L_{Q|vw}(z+\tau i a Q )\right) H(z+\tau Ma-u).
\eea
Combining all the terms with $\Lambda_{\pm}$ from \eqref{92v} and \eqref{93v} gives:
\bea
&-& \left(\int_{(-\pi,\pi)+i\e}-\int_{(-\pi,\pi)-i\e}\right)\left(\Lambda_-(z) H(z+M a i -u) + \Lambda_-(z) H(z-M a i -u)\right) \nn
&-&\sum_{\tau} \tau \int_{(-\pi,\pi) -i\tau \e }\left(\Lambda_--\Lambda_+ \right) H(z+\tau M a-u).
\eea
Using the relation
\bea
\int_{(-\pi,\pi) \pm i \e} (r -r*) f = \oint_{\gamma_0} r f\pm \oint_{\gamma_x} r f,
\eea
for an analytic function $f$, a function $r$ with square root branch cuts and the contours $\gamma_0$ and $\gamma_x$ defined in Extended $Y$-system on the finite interval, we can rewrite this expression for $Y_-$'s as 
\bea
\left(\Lambda_--\Lambda_+\right) \hat{\star} K_M. 
\eea
Collecting all the remaining terms and plugging in the relation from \eqref{Didentityv} into the first line leads to
\bea
\label{derivvw1}
 &-& \sum_{\tau}\sum_{l=1}^{\infty}\tau  \int_{(-\pi,\pi) -i\tau \e }H(z+\tau (M+2l)ai-u)\cdot  \nn
& &\, \left(L_{l|vw}(z+\tau li a)+L_{M+l|vw}(z+\tau (M+l)i a) +2 \sum_{Q=l+1}^{M-1+l}  L_{Q|vw}(z+\tau Qi a)-\sum_{Q=1+l}^{M+l} \Lambda_Q(z+\tau Qai)\right)\nn
&+& \sum_{Q=1}^{M-1} L_{Q|vw}\star K_{M-Q},
\eea
which contains a lot of familiar terms. In fact, only the summation over $\Lambda_Q$ is new. Therefore, we can only treat this new part and use the result for the remaining terms as we calculated it in the derivation of the TBA-equation for $Y_w$: 
\bea
&-& \sum_{\tau}\sum_{l=1}^{\infty}\tau  \int_{(-\pi,\pi) -i\tau \e }H(z+\tau (M+2l)ai-u)\cdot  \nn
& &\qquad \left(L_{l|vw}(z+\tau li a)+L_{M+l|vw}(z+\tau (M+l)i a) +2 \sum_{Q=l+1}^{M-1+l}  L_{Q|vw}(z+\tau Qi a)\right)+ \sum_{Q=1}^{M-1} L_{Q|vw}\star K_{M-Q} \nn
&=& \sum_{l=1}^{\infty} L_{l|vw} \star \left( 2\sum_{Q=1}^{\min(M,l)-1} K_{|M-l|+2Q} +  K_{|M-l|} +  K_{M+l} \right) = \sum_{l=1}^{\infty} L_{l|vw} \star K_{lM}.
\eea
So in order to find the TBA-equation, we need to simplify the term \marginnote{\checkmark Mma}
\bea
& & \sum_{\tau}\sum_{l=1}^{\infty}\tau  \int H(z+\tau (M+2l)ai-u)\sum_{Q=1+l}^{M+l} \Lambda_Q(z+\tau Qai) \nn
&=& \sum_{\tau}\sum_{l=1}^{\infty}\tau  \int H(z+\tau (M+2l-Q)ai-u)\sum_{Q=1+l}^{M+l} \Lambda_Q(z) \nn
&=& - \sum_{l=1}^{\infty} \sum_{Q=1+l}^{M+l} \Lambda_Q\star K_{M+2l-Q} \nn
&=& -\sum_{Q=1}^{\infty}  \sum_{l=\max(M-Q,0)}^{M-1}  \Lambda_{Q+1}\star K_{Q+1+2l-M},
\eea
after shifting $l\rightarrow l+Q-M$. Our total right-hand side for the the TBA-equation of $Y_{M|vw}$ (with $M\geq 2$) now reads
\bea
\sum_{N=1}^{\infty} L_{N|vw} \star K_{NM} + \left(\Lambda_--\Lambda_+\right) \hat{\star} K_M-\sum_{Q=1}^{\infty}  \sum_{l=\max(M-Q,0)}^{M-1}  \Lambda_{Q+1}\star K_{Q+1+2l-M}. 
\eea
Changing the $\Lambda_{\beta}$'s into $L_{\beta}$'s and using the TBA-equation for $Y_{\beta}$ yields
\bea
\sum_{N=1}^{\infty} L_{N|vw} \star K_{NM} + \left(L_--L_+\right) \hat{\star} K_M-\sum_{Q=1}^{\infty} L_Q\star K_{Qy}\hat{\star}K_M-\sum_{Q=1}^{\infty}  \sum_{l=\max(M-Q,0)}^{M-1}  \Lambda_{Q+1}\star K_{Q+1+2l-M}. 
\eea
Gathering all the terms depending on $Y_Q$'s gives us
\bea
-\sum_{Q=1}^{\infty} L_Q\star \left( K_{Qy}\hat{\star}K_M+(1-\delta_{Q,1}) \sum_{l=\max(M-Q+1,0)}^{M-1}  K_{Q+2l-M}\right)
\eea
and using the fact that the terms in the brackets sum up to exactly $K_{xv}^{QM}$ we find the TBA-equation for $Y_{vw}$: \marginnote{Kernel identity checked numerically in Mma}
\bea
\log Y_{M|vw} = L_{N|vw} \star K_{NM} +\left(L_--L_+\right) \hat{\star} K_M-\Lambda_Q \star K_{xv}^{QM}.
\eea
To finish of this section we need to check two things: first we have to do the computation for $M=1$ and second we have to check the fact that the brackets in the second to last equation sum up to $K_{xv}^{QM}$. Checking the identity for the kernels can be done numerically in Mathematica, which was done successfully in the usual notebook for $1\leq Q,M \leq 10$ and arbitrary real numbers for the other variables. To see that our derivation also works for $M=1$ we remark that the expression \eqref{rep2v} is also valid for $M=1$, after which the rest of the derivation works for all $M\in \mathbb{N}$. In particular we see that the same holds for the $Y_w$, for which we only need to remove the dependence on $\Lambda_Q$'s. 
\\[5mm]
We would like to provide a proof of the kernel identity used in the last lines above. 

==> kernelsandenergies.tex <==
The kernels that appear in the TBA-equations \eqref{TBAeqns} are defined as follows:
\be
K_M (u) = \frac{1}{2\pi} \frac{ \sinh M\ad}{\cosh M\ad- \cos u}
\ee
\be
K_{MN} (u) = K_{M+N} (u)+ K_{|M-N|} (u)+2\sum_{j=1} ^{\min(M,N)-1} K_{|M-N|+2j} (u)
\ee
The other kernels are defined directly from the scattering matrices
\bea
S_-^{yQ}(u,v) &=& q^{Q/2} \frac{x(u) - x^+(v) }{x(u) - x^-(v) }\sqrt{\frac{x^+(v)}{x^-(v)}} \\
S_+^{yQ}(u,v) &=& q^{Q/2} \frac{1/x(u) - x^+(v) }{1/x(u) - x^-(v) }\sqrt{\frac{x^+(v)}{x^-(v)}} \\
S_-^{Qy}(u,v) &=& q^{Q/2} \frac{x^-(u) - x(v) }{x^+(u) - x(v) }\sqrt{\frac{x^+(u)}{x^-(u)}} \\
S_+^{Qy}(u,v)& =& q^{Q/2} \frac{x^-(u) - 1/x(v) }{x^+(u) - 1/x(v) }\sqrt{\frac{x^+(u)}{x^-(u)}}\\
S_{xv}^{QM}(u,v) &=& q^{Q} \frac{x^-(u) - x^{+M}(v) }{x^+(u) - x^{+M}(v) } \frac{x^-(u) - x^{-M}(v) }{x^+(u) - x^{-M}(v) }\frac{x^+(u)}{x^-(u)} \prod_{j=1}^{M-1} S_{Q+M-2j}(u-v) ,
\eea
where $x^{\pm}(v) = x(v\pm i Q \ad)$, $x^{\pm M}(v) = x(v\pm i M \ad)$ and 
\be
S_{Q}(u) = \frac{\sin \frac{1}{2} (u-i Q \ad)}{\sin \frac{1}{2} (u+i Q \ad)}.
\ee
They are given by
\bea
K_{xv}^{QM}(u,v) = \frac{1}{2\pi i} \frac{d}{du} \log S_{xv}^{QM} (u,v) \\
K_{vwx}^{MQ}(u,v) = -\frac{1}{2\pi i} \frac{d}{du} \log S_{xv}^{QM} (v,u) \\
K_{\beta}^{Qy}(u,v) = \frac{1}{2\pi i} \frac{d}{du} \log S_{\beta}^{Qy} (u,v) \\
K_{\beta}^{yQ}(u,v) = \beta \frac{1}{2\pi i} \frac{d}{du} \log S_{\beta}^{Qy} (v,u)
\eea
and finally the dressing phase kernel
\be
K^{PQ}_{\mathfrak{sl}(2)}(u,v) = \frac{1}{2\pi i} \frac{d}{du} \log S^{PQ}_{\mathfrak{sl}(2)},
\ee
where we refrain from explicitly writing down expressions for the scattering matrix due to its complexity (see \cite{} for explicit expressions). \marginnote{I guess this is Hoare Hollowood etc.}
\\[5mm]
Some important identities for the kernels are
\bea
\label{kernelids}
K_{Qy}(u,v) &\defeq& K_{-}^{Qy}(u,v)-K_{+}^{Qy}(u,v)  = K(u+ i Q \ad,v) -K(u- i Q\ad,v) \\
K_{yQ}(u,v) &\defeq& K_{-}^{yQ}(u,v)+K_{+}^{yQ}(u,v)  = K(u,v- i Q \ad) -K(u,v+ i Q \ad) \\
K_{-}^{yQ}(u,v) - K_{+}^{yQ}(u,v) &=& K_{-}^{Qy}(u,v)+K_{+}^{Qy}(u,v)  = K_Q(u-v),
\eea
with the kernel
\be
K(u,v) = \frac{1}{2\pi i} \frac{d}{du} \log\frac{x(u) - 1/x(v) }{x(u) - x(v) }.
\ee
We can define the similar kernel 
\be
\bar{K}(u,v) = \theta\left(|u|-\theta \right) \frac{1}{2\pi i} \frac{d}{du} \log\frac{x(u) - 1/x_s(v) }{x(u) - x_s(v) }
\ee
and the associated 
\be
\widecheck{K}_{M}(u,v)  = \bar{K}(u+ i M \ad,v) +\bar{K}(u- i M \ad,v).
\ee
The mirror energy and momentum are defined through the $x$-functions as follows:
\be
\label{eq:mirrormomentum}
 \tilde{p}^Q = \frac{i}{\ad}\log \left( q^Q \frac{x^+}{x^-}\frac{x^-+\xi}{x^++\xi}\right), \quad \tilde{E}_Q= -\log \left( \frac{1}{q^Q}\frac{x^++\xi}{x^-+\xi}\right). 
\ee


==> preambletikz.tex <==
\usepackage{tikz}
\usetikzlibrary{calc,shapes,backgrounds}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.markings}

\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

\tikzset{middlearrow/.style={
        decoration={markings,
            mark= at position 0.5 with {\arrow{#1}} ,
        },
        postaction={decorate}
    }
}

\usepackage{xcolor}
\colorlet{MyColorOne}{black!100}

\newcommand{\lightercolor}[3]{% Reference Color, Percentage, New Color Name
    \colorlet{#3}{#1!#2!white}
}
\lightercolor{MyColorOne}{40}{MyColorOneLight}
\lightercolor{MyColorOne}{10}{MyColorOneLightest}
\lightercolor{MyColorOne}{5}{MyColorOneLightest2}
